Reinforcement Learning-Based REST API Testing with Multi-Coverage

REST (Representational State Transfer) APIs have become integral for data communication and exchange due to their simplicity, scalability, and compatibility with web standards. However, ensuring REST APIs' reliability through rigorous testing poses significant challenges, given the complexities of operations, parameters, inputs, dependencies, and call sequences. In this paper, we introduce MUCOREST, a novel Reinforcement Learning (RL)-based API testing approach that leverages Q-learning to maximize code coverage and output coverage, thereby improving bug discovery. By focusing on these proximate objectives rather than the abstract goal of maximizing failures, MUCOREST effectively discovers critical code areas and diverse API behaviors. The experimental results on a benchmark of 10 services show that MUCOREST significantly outperforms state-of-the-art API testing approaches by 11.6-261.1% in the number of discovered API bugs. MUCOREST can generate much fewer API calls to discover the same number of bugs compared to the other approaches. Furthermore, 12.17%-64.09% of the bugs discovered by the other techniques can also be found by MUCOREST.

==> 3.backup.tex <==
\section{Approach \label{approach}}

This section describes, \tool, our novel RL-based API testing approach, which is designed to discover API bugs. In \tool, this long-term goal is pursued through two immediate objectives in discovering API bugs: maximizing the code coverage and maximizing output coverage.
%
% o achieve this goal establish guidelines that will expand the diversity of API responses and maximize both output and code coverage. 
We model the task of discovering API bugs as a RL task. Specifically, in \tool, the \textit{system under test} serves as the \textit{environment} and the \textit{agent} is responsible for generating API calls and executing the calls. The \textit{state} is expressed via current code coverage, output coverage, and other state variables, and the \textit{actions} include selecting operations and input parameters to form API calls. The \textit{reward} is determined by evaluating the code coverage, output coverage, and API call's response.

% Initially, essential elements are initialized for the Q-learning process, followed by the prioritization mechanism that determines the best operations and value mappings. Upon obtaining SUT feedback, we evaluate the outcomes to calculate the rewards derived from the agent’s actions and proceed to update the Q-Table.


%SON COMMENT OUT
% The reward system operates based on the quality of output and the code coverage achieved. Our analysis of the output, especially the API responses as well as code coverage, is conducted from three distinct perspectives. The first perspective seeks to assign rewards that reflect the possibility of detecting erroneous behavior, incorporating its response status code. The second angle focuses on rewarding the uniqueness of the response, where a novel reply indicates new output and access to previously untouched code segments, thereby incrementally gaining the SUT's output and code coverage. Conversely, repeated identical responses and status codes indicate a deadlock in progress. Finally, we utilize code coverage metrics as an additional viewpoint to get a deeper insight into the testing process and its effectiveness.
% In the following, we will detail the two critical components of \tool, i.e., output coverage, and code coverage as well as different attributes of each part.

\subsection{Q-learning Algorithm for RL-based API Testing}

In this work, we reuse the basic components of Q-learning Algorithm in ARAT-RL~\cite{arat}. Figure \ref{img:arat-rl-workflow} provides an overview of the ARAT-RL approach, which consists of three main stages.
In the first stage, Q-Learning Table Initialization, ARAT-RL initializes the Q-table by analyzing parameter usage frequency in operations and prioritizing common parameters for early examination. It includes various input sources for flexibility and tracks their performance in a separate Q-table to optimize input selection for future tests. In Q-Learning-based prioritization, test case inputs are created through three steps: $SelectOperation$, $SelectParameters$, and $SelectValueMappingSource$. Choices are made using an $\epsilon$-greedy policy; if a random value is above $\epsilon$, the highest Q-value source is chosen, otherwise, a random source is selected. This strategy prevents settling for suboptimal solutions by exploring various sources. Finally, ARAT-RL updates the Q-table after test case execution, decreasing Q-values for successful responses (2xx) and increasing them for failed requests (4xx or 5xx), aiding in the testing of various API operations and parameters.

\begin{figure}[htp]
	\includegraphics[width=1\columnwidth]{figures/Workflow_ARAT-rl.drawio.png}
	\centering
	\caption{Workflow of ARAT-RL.}
	\label{img:arat-rl-workflow}
\end{figure}

% \textbf{Q-Learning Table Initialization.} In the first phase, ARAT-RL constructs the initial state of the Q-table by analyzing the frequency of parameter usage for each operation in the specification. It prioritizes frequently appearing parameters as they might hold greater importance. Thereby, operations composed of these parameters are examined in advance. Besides, to enhance flexibility in test cases, ARAT-RL also incorporates diverse input value sources for the operations. Another Q-table is created to track the performance scores of each source. This helps ARAT-RL select the most effective input source for subsequent test iterations.

% \textbf{Q-Learning-based Prioritization.} For the creation of test case inputs, three essential procedures need to be conducted: $SelectOperation$, $SelectParameters$, and $SelectValueMappingSource$. Each selection procedure in the learning phase is guided based on the $\epsilon$-greedy policy. If a randomly generated value surpasses $\epsilon$, the algorithm opts for the source with the highest Q-value for the chosen operation. Otherwise, the algorithm proceeds to select an arbitrary source from the available options. This randomness ensures that the algorithm occasionally explores less promising mapping sources to avoid reaching a suboptimal solution.

% \textbf{Q-Learning-based API Testing.} Since the creation and execution of test cases, ARAT-RL updates the Q-table based on the response status codes. A successful status code (\texttt{2xx}) prompts ARAT-RL to lower the Q-values. Conversely, a status code denoting a request failure (\texttt{4xx} or \texttt{5xx}) leads to an increment in the Q-values. This mechanism enables the Reinforcement Learning model to test diverse API operations and their associated parameters.

% The ARAT-RL’s Q-Learning approach shows potential but is constrained by its dependence on API status codes, which doesn’t fully exploit the feedback from the SUT. Using more details from the response’s structure and novelty, among other factors, could significantly boost the Reinforcement Learning strategy’s performance. Solely relying on the response status codes may lead to suboptimal output coverage and a reduced capacity for identifying possible API errors.

% \textbf{Outstanding Issues.} While ARAT-RL  Reinforcement Learning efficiently and shows promise, its Q-Learning update strategy responsible for reward assessment has notable shortcomings in fully exploiting SUT's feedback. This strategy primarily depends on the response status codes from the API, neglecting additional informative data that could refine the learning and optimization processes. Incorporating insights from the response’s structure and uniqueness, among other aspects, could significantly improve the Reinforcement Learning strategy’s effectiveness. Relying solely on the response status codes may lead to suboptimal output coverage and a diminished capacity for identifying possible API errors.

\subsection{Output coverage}

% During API quality assurance, an operation’s result is demonstrated as an HTTP response, with the response status code indicating the success or failure of the operation. While each status code conveys a specific message, we have organized them into four categories, each reflecting a distinct degree of contribution to the testing phase.

% \textit{401 (Unauthorized), 403 (Forbidden).} These status codes indicate permission issues, resulting in denied access to the API resources. Such responses are not useful for testing since the SUT has not performed any action on the API resources, leaving us without actionable data.

% \textit{4xx, 3xx, and 2xx.} An expected state of the SUT is reflected by this group of status codes. They confirm that certain source code blocks were executed, providing feedback on the success or failure of the action.

% \textit{5xx.} A status code in the 500 range points to internal errors within the SUT during request processing. Although it represents an undesirable outcome of an API call, it is also the most informative for API Testing purposes.

% \textit{No response.} The absence of any response from an API call is highly problematic, both during testing and in production environments. A lack of response offers no clues about the SUT’s operational status or potential network issues.



\textbf{Evaluating reward based on status code.} Response status codes serve as indicators of expected results during API testing. Certain codes confirm the test’s effectiveness, while others suggest less productive test strategies. Therefore, we categorize these codes into four groups to reflect their varying levels of impact on the testing process.
% Therefore, we will evaluate the reward based on the expected appearance of a response status code within the groups of status codes categorized above.

    \textit{401 (Unauthorized), 403 (Forbidden).} Endpoints that are off-limits due to authentication or authorization issues should not be encountered during testing. To conserve resources and optimize rewards, it is advisable to refrain from repeated testing of such endpoints, as this typically leads to lowering the reward.
    
    \textit{4xx, 3xx, and 2xx.} These status codes enhance the breadth of output coverage. While they do not significantly advance the identification of bugs, their discovery warrants a minor increase in rewards.
    % Furthermore, when these codes are absent from the official specification, an additional reward is granted. Undocumented status code often stems from errors in source code that lack corresponding specifications. Discovering code that extends beyond the documented specifications can be deemed innovative; however, since it does not directly correlate with the bug detection process, a minimal reward is issued.
    
    \textit{5xx.} In API testing, the 5xx status code is a key focus area. The detection of 5xx errors indicates the discovery of a new bug, which is considered a significant finding and is thus rewarded generously.
    
    \textit{No response.} The lack of responses could be due to server overload, slow code execution, or bugs. To prevent server issues, stop testing the endpoint temporarily, which may lead to reduced rewards. This restriction may be momentary, permitting future retests of the endpoint during the testing period.
    % The lack of a response can stem from various causes such as server overload, slow processing of the source code resulting in timeouts, or the existence of bugs hindering the return of a response. To prevent server strain, it is advisable to cease testing the endpoint, leading to a decrease in the reward. However, this restriction might be temporary, allowing for the possibility of retesting the endpoint later during the testing phase.
    % While penalties are imposed, they are not as severe as those for 401 and 403 errors because retesting is anticipated.
    % On the other hand, problems such as unexpected behaviors, potentially including fraud, may occur. Nonetheless, the absence of a response limits further exploitation of information, and the model cannot learn from these requests. The standard approach for instances with no response is to discontinue testing the endpoint by reducing the reward
    % , but to a lesser extent than for 401 and 403 errors and recording the requests causing timeouts for subsequent manual review.

 \textbf{Evaluating reward based on response novelty.} Rewards are determined with an emphasis on the uniqueness of responses. The preliminary objective is to expand output coverage by rewarding new or infrequent responses.
 % Responses that recur frequently are deemed routine.
 For instance, a 5xx status code response indicates a server error but loses its significance if it is a common occurrence. Analyzing routine responses helps reduce unnecessary requests and improve test efficiency. The initial reward, derived from the status code analysis, forms the groundwork for the subsequent reward estimation. A coefficient, denoted as $d$, is used to highlight the uniqueness of a response. The final reward is calculated by multiplying the initial score by $d$ to reflect the response’s novelty. \begin{equation}
    reward_{novelty} = reward_{status\_code} \times d
\end{equation}

Assessing a response’s innovation is done by comparing it with the $k$ closest historical responses sharing the same operation and status code. This comparison determines if and how closely the current response aligns with historical ones. The coefficient $d$, reflecting response novelty, is calculated accordingly and varies for the four specific response status code scenarios previously outlined.

% The similarity between two responses can result in two cases:
% \begin{itemize}
%     \item Either an absolute match or mismatch - absolute comparison
%     \item Different levels of similarity, using a score to evaluate the degree of similarity - relative comparison
% \end{itemize}
% Depending on the status code and response body, we can either make an absolute or relative comparison between the two responses.

 \textit{No response and 401 (Unauthorized), 403 (Forbidden).} To prevent additional testing of endpoints that yield no beneficial responses, it is unnecessary to examine the $k$ closest responses. The reward is preserved at its current level by maintaining the coefficient $d$ at a constant value of $1$.

\textit{5xx, 4xx, 3xx, and 2xx.} A response with any of these status codes indicates active SUT functionality. However, repeated identical error codes don’t aid testing. The idea is to examine the current response's body against the last $k$ responses with the same operation and status code in the history. A unique response may indicate a new issue and grant a high reward.

%         \begin{itemize}
%             \item Step 1. Check the response novelty: Compare the stack trace of the current response with all historical stack traces. If no matching stack trace is found, concluding a new bug and bypassing Step 2.
%                 
%             \item Step 2. Check the response duplication: Compare the $k$ most recent responses of the same type.                   
%         \end{itemize}
%     \item \texttt{4xx}, \texttt{3xx} and \texttt{2xx}: The responses fall into one of four categories: no response returned, error message returned, successful message returned, or successful response body returned.
%         \begin{itemize}   
%         \item Step 1. Check the novelty of the response status code: If the response status code is not found in the test history, it indicates a novel response. Otherwise, move on to step 2.
%         \item Step 2. Check the response duplication by one of the following methods depending on the response type:
%             \begin{itemize}
%                 \item Comparing the message and body.
%                 \item Comparing the structure of two response bodies.
%                 \item Comparing with the $k$ most recent responses of the same type.
%             \end{itemize}
%         \end{itemize}

\subsection{Code coverage}

API testing often relies on responses, but having the source code can offer extra insights. The method in the previous section that exclusively uses output coverage is known as black-box testing, which can be effective. However, including code coverage data, though not mandatory, can greatly improve test results. We recommend combining code coverage as a complement to output coverage to enhance the testing outcomes.

% API testing often depends on the response received. Nonetheless, under certain circumstances, when source code is available, thereby unlocks beneficial resources. The methodologies that exclusively utilize the output are denominated as black-box testing, such as the approach described in the previous section, which can still produce appropriate outcomes for the testing procedure. The integration of supplementary data regarding code coverage, while not mandatory, can enhance the output coverage. We intend to advocate the adoption of code coverage as a complement to output coverage. This integration aims to enhance the reward evaluation framework, ultimately leading to more advantageous outcomes within the testing paradigm.

\textbf{Evaluating reward based on code coverage.} Our goal is to guide the agent to explore untested areas of the API by tracking the code paths that each request executes. Requests that cover new parts of the source code receive higher rewards, promoting the agent to interact with diverse API functions. Evaluating responses solely through black-box testing can overlook scenarios where identical outputs may arise from different segments of code. Therefore, it’s crucial to include other considerations besides the response when assessing outputs.

Manipulating the source code is essential for obtaining code coverage metrics, hence this approach is identified as grey-box testing. This method assesses code coverage gains by tracking the number of new lines of code executed per request. Rewards are allocated in proportion to the additional lines of code executed relative to the total source code. However, it’s important to balance the significance of newly executed lines against the overall code coverage, which unfolds in three testing stages of the testing cycle. In the initial stage, an initial spike in code coverage is expected, therefore the incentive for gaining code coverage is relatively small. As progress in the middle phase, the increment in newly executed lines of code gradually decreases towards zero, leading to a minimal rise in code coverage. Finally, it is common for new code execution along with overall code coverage's increment to stabilize at zero when reaching saturation. Nonetheless, certain requests can lead to a surprising boost in code coverage by triggering code segments that have not been previously executed. Requests that unexpectedly increase coverage, especially during saturation, deserve significant rewards.

% Employing code coverage as a guide for making test decisions is key to addressing scenarios such as the following:
% Employing code coverage as a guide for making test decisions is key to addressing such scenarios

% \begin{itemize}
%     \item Different code segments are being executed but producing the same output.
%     \item Situations where the output is too limited or lacks sufficient information. For example, if the response message consistently returns the same message for different failure actions, it becomes infeasible to distinguish previous and subsequent responses.
% \end{itemize}



% The starting point of round 2 will be distinct from round 3. The formula for the total reward points will be:
% \begin{equation}
%     reward_{total} = reward_{r2}(reward_{output\_coverage}) + reward_{r3}(reward_{code\_coverage})
% \end{equation}

% Workflow \\
% 2 things: Output coverage, code coverage \\
% 3 round, 1 2 out coverage, 3 code coverage \\
